Prompt Problems: A New Programming Exercise for the Generative AI Era

Large Language Models (LLMs) are revolutionizing the field of computing education with their powerful code-generating capabilities. Traditional pedagogical practices have focused on code writing tasks, but there is now a shift in importance towards code reading, comprehension and evaluation of LLM-generated code. Alongside this shift, an important new skill is emerging -- the ability to solve programming tasks by constructing good prompts for code-generating models. In this work we introduce a new type of programming exercise to hone this nascent skill: 'Prompt Problems'. Prompt Problems are designed to help students learn how to write effective prompts for AI code generators. A student solves a Prompt Problem by crafting a natural language prompt which, when provided as input to an LLM, outputs code that successfully solves a specified programming task. We also present a new web-based tool called Promptly which hosts a repository of Prompt Problems and supports the automated evaluation of prompt-generated code. We deploy Promptly for the first time in one CS1 and one CS2 course and describe our experiences, which include student perceptions of this new type of activity and their interactions with the tool. We find that students are enthusiastic about Prompt Problems, and appreciate how the problems engage their computational thinking skills and expose them to new programming constructs. We discuss ideas for the future development of new variations of Prompt Problems, and the need to carefully study their integration into classroom practice.

==> notes.tex <==
In figures>promptproblem-why-not.png, 

-----
[via "myFunc" produce twice the input ]

ChatGPT response:

function myFunc(num) {
  return num * 2;
}

Code Running response:

Traceback (most recent call last):
  File "/home/jobe/runs/jobe_KjrkW8/test.c", line 3, in <module>
    myFuncmyFunc
NameError: name 'myFuncmyFunc' is not defined
-----

Question:  it says "You pass!" but is that wrong given the "ChatGPT response" ?

[double input number 'myFunc']

ChatGPT response:

MyFunc is not a valid input. Please enter a valid number.

Code Running response:

You pass!
-----

In figures>promptproblem-oops-1.png
"You pass!", but function is:

function myFunc(x, y) { return x * 2 + y * 2; }

\begin{figure}
\centering
  \includegraphics[scale=0.3125]{figures/promptproblem-oops-1.png}
  \caption{oops-1}
  \label{fig:prompt-problem-oops-1}
\end{figure}


begin{itemize}
  \item will social student games arise?  "Bet I can name that tune in 7 words."  "Hah! I can do it in 6."
  \item future(?) problem description has "include some of these words". then 7 words are shown, but only 3 are relevant.  Student has to figure our which are the relevant words.
  \item future(?) Or "for a hint, click here" then successively more/better words are revealed.  Possibly losing points each time.
  \item future(?) "team competition" 2-4 people sitting next to each other and yelling out the words they are trying, in parallel so that more words can be tried quicker.
\end{itemize}


% Busjahn, Schulte, "Analysis of Code Reading to gain more Insight in Program Comprehension"
% Code reading, although an integral part of program comprehension, is rarely reflected. In this paper, we want to argue for a research approach and direction exploiting the potential that lies in the analysis of reading processes. Based on the vast experience compiled in psychology and some studies in computing, eye tracking and think aloud were elaborated as a viable research instrument for code reading studies. We conducted a feasibility study, designed to examine the actual process of code reading as the sensory starting point of comprehension. Computational and statistical tools were developed to facilitate data capture and analysis for eye tracking experiments. 
% Results do not just provide proof of concept but already emphasize differences between reading natural language text and source code, as well as a distinct attention allocation within different code elements like keywords and operators.
% In conclusion we suggest a combination of theory-driven selected stimuli material, a carefully designed procedure of eye tracking, complemented with suitable post-tests on comprehension as well as retrospective think aloud in order to obtain additional information on the linking process between perception and comprehension. As an addition to other research approaches this should most certainly help us to improve our knowledge of comprehension within an educational research framework

The DOT language of graphviz (https://graphviz.org/) is an example of how graphical models can be represented textually.  Having visual and textual representations... can help make for interesting testing.
For example, a UML diagram can be shown and the student can be asked to create prompts that will guide the LLM in generating the DOT language text that creates such a diagram.

-----

"constant progress" nope. continued, non-stop, unrelenting.
"era" drama.  development, iteration, step
can an abstract have a "for example" ?
'read, understand, evaluate' - is there a delta? a - or +?
'is likely to become' is becoming.  SQL _did_ entirely replace "database coding"

we used to teach everything, knowing some of it only a few would use, but all allegedly benefited from learning.  do we finally officially give up on that?

are spreadsheets like python-vs-c (indent/visual has meaning like column 3)?
does python manage hierarchy _differently_ from {}?
vs C, do syntax/semantic errors differ as python _forces_ indentation, i.e, when I get to choose how a thing looks, I "am deciding" as I go a long, but with Python I am not deciding the look.  Surely a slightly different part of the brain is lighting up?  How about eye-tracking study?


